On the Enumeration of Maximal $(\Delta, \gamma)$-Cliques of a Temporal Network

A temporal network is a mathematical way of precisely representing a time varying relationship among a group of agents. In this paper, we introduce the notion of $(\Delta, \gamma)$-Cliques of a temporal network, where every pair of vertices present in the clique communicates atleast $\gamma$ times in each $\Delta$ period within a given time duration. We present an algorithm for enumerating all such maximal cliques present in the network. We also implement the proposed algorithm with three human contact network data sets. Based on the obtained results, we analyze the data set on multiple values of $\Delta$ and $\gamma$, which helps in finding out contact groups with different frequencies.

==> bare_conf_ <==
@article{bron1973algorithm,
  title={Algorithm 457: finding all cliques of an undirected graph},
  author={Bron, Coen and Kerbosch, Joep},
  journal={Communications of the ACM},
  volume={16},
  number={9},
  pages={575--577},
  year={1973},
  publisher={ACM}
}

@inproceedings{cheng2012fast,
  title={Fast algorithms for maximal clique enumeration with limited memory},
  author={Cheng, James and Zhu, Linhong and Ke, Yiping and Chu, Shumo},
  booktitle={Proceedings of the 18th ACM SIGKDD international conference on Knowledge discovery and data mining},
  pages={1240--1248},
  year={2012},
  organization={ACM}
}

@article{eppstein2011listing,
  title={Listing all maximal cliques in large sparse real-world graphs},
  author={Eppstein, David and Strash, Darren},
  journal={Experimental Algorithms},
  pages={364--375},
  year={2011},
  publisher={Springer}
}

@article{eppstein2013listing1,
  title={Listing all maximal cliques in large sparse real-world graphs},
  author={Eppstein, David and L{\"o}ffler, Maarten and Strash, Darren},
  journal={Journal of Experimental Algorithmics (JEA)},
  volume={18},
  pages={3--1},
  year={2013},
  publisher={ACM}
}

@article{holme2012temporal,
  title={Temporal networks},
  author={Holme, Petter and Saram{\"a}ki, Jari},
  journal={Physics reports},
  volume={519},
  number={3},
  pages={97--125},
  year={2012},
  publisher={Elsevier}
}

@inproceedings{viard2015revealing,
  title={Revealing contact patterns among high-school students using maximal cliques in link streams},
  author={Viard, Jordan and Latapy, Matthieu and Magnien, Cl{\'e}mence},
  booktitle={Proceedings of the 2015 IEEE/ACM International Conference on Advances in Social Networks Analysis and Mining 2015},
  pages={1517--1522},
  year={2015},
  organization={ACM}
}

@article{viard2016computing,
  title={Computing maximal cliques in link streams},
  author={Viard, Tiphaine and Latapy, Matthieu and Magnien, Cl{\'e}mence},
  journal={Theoretical Computer Science},
  volume={609},
  pages={245--252},
  year={2016},
  publisher={Elsevier}
}

@inproceedings{himmel2016enumerating,
  title={Enumerating maximal cliques in temporal graphs},
  author={Himmel, Anne-Sophie and Molter, Hendrik and Niedermeier, Rolf and Sorge, Manuel},
  booktitle={Advances in Social Networks Analysis and Mining (ASONAM), 2016 IEEE/ACM International Conference on},
  pages={337--344},
  year={2016},
  organization={IEEE}
}

@article{mukherjee2017enumeration,
  title={Enumeration of maximal cliques from an uncertain graph},
  author={Mukherjee, Arko Provo and Xu, Pan and Tirthapura, Srikanta},
  journal={IEEE Transactions on Knowledge and Data Engineering},
  volume={29},
  number={3},
  pages={543--555},
  year={2017},
  publisher={IEEE}
}

@inproceedings{mukherjee2015mining,
  title={Mining maximal cliques from an uncertain graph},
  author={Mukherjee, Arko Provo and Xu, Pan and Tirthapura, Srikanta},
  booktitle={Data Engineering (ICDE), 2015 IEEE 31st International Conference on},
  pages={243--254},
  year={2015},
  organization={IEEE}
}

@book{holme2013temporal,
  title={Temporal networks},
  author={Holme, Petter and Saram{\"a}ki, Jari},
  year={2013},
  publisher={Springer}
}


@MISC{konect:2016:mit,
    title = {Reality Mining network dataset -- {KONECT}},
    month = sep,
    year = {2016},
    url = {http://konect.uni-koblenz.de/networks/mit}
}

@article{konect:eagle06,
        title = {{Reality} {Mining}: Sensing Complex Social Systems}, 
        author = {Eagle, Nathan and (Sandy) Pentland, Alex},
        journal = {Personal Ubiquitous Computing},
        volume = {10},
        number = {4},
        year = {2006},
        pages = {255--268},
}


@inproceedings{konect,
	title = {{KONECT} -- {The} {Koblenz} {Network} {Collection}},
	author = {Jérôme Kunegis},
	year = {2013},
	booktitle = {Proc. Int. Conf. on World Wide Web Companion},
	pages = {1343--1350},
	url = {http://userpages.uni-koblenz.de/~kunegis/paper/kunegis-koblenz-network-collection.pdf}, 
	url_presentation = {http://userpages.uni-koblenz.de/~kunegis/paper/kunegis-koblenz-network-collection.presentation.pdf},
}

@MISC{konect:2017:sociopatterns-infectious,
    title = {Infectious network dataset -- {KONECT}},
    month = apr,
    year = {2017},
    url = {http://konect.uni-koblenz.de/networks/sociopatterns-infectious}
}

@article{konect:sociopatterns,
	author = {Lorenzo Isella and Juliette Stehlé and Alain Barrat and Ciro
                  Cattuto and Jean-François Pinton and Wouter Van den
                  Broeck}, 
	title = {What's in a Crowd? Analysis of Face-to-Face Behavioral Networks},
	journal = {J. of Theoretical Biology},
	volume = {271},
	number = {1},
	pages = {166--180},
	year = {2011},
}

@article{johnson1988generating,
	title={On generating all maximal independent sets},
	author={Johnson, David S and Yannakakis, Mihalis and Papadimitriou, Christos H},
	journal={Information Processing Letters},
	volume={27},
	number={3},
	pages={119--123},
	year={1988},
	publisher={Elsevier}
}

@book{masuda2017temporal,
  title={Temporal Network Epidemiology},
  author={Masuda, Naoki and Holme, Petter},
  year={2017},
  publisher={Springer}
}

@article{hulovatyy2015exploring, 
title={Exploring the structure and function of temporal networks with dynamic graphlets}, 
author={Hulovatyy, Yuriy and Chen, Huili and Milenkovi{\'c}, T}, 
journal={Bioinformatics}, 
volume={31}, 
number={12}, 
pages={i171--i180}, 
year={2015}, 
publisher={Oxford University Press} 
}

@book{garey2002computers,
  title={Computers and intractability},
  author={Garey, Michael R and Johnson, David S},
  volume={29},
  year={2002},
  publisher={wh freeman New York}
}

@article{chaintreau2007impact,
  title={Impact of human mobility on opportunistic forwarding algorithms},
  author={Chaintreau, Augustin and Hui, Pan and Crowcroft, Jon and Diot, Christophe and Gass, Richard and Scott, James},
  journal={IEEE Transactions on Mobile Computing},
  volume={6},
  number={6},
  pages={606--620},
  year={2007},
  publisher={IEEE}
}

@article{panzarasa2009patterns,
  title={Patterns and dynamics of users' behavior and interaction: Network analysis of an online community},
  author={Panzarasa, Pietro and Opsahl, Tore and Carley, Kathleen M},
  journal={Journal of the Association for Information Science and Technology},
  volume={60},
  number={5},
  pages={911--932},
  year={2009},
  publisher={Wiley Online Library}
}

